As time goes by: Constraint Handling Rules - A survey of CHR research from 1998 to 2007

Constraint Handling Rules (CHR) is a high-level programming language based on multi-headed multiset rewrite rules. Originally designed for writing user-defined constraint solvers, it is now recognized as an elegant general purpose language. CHR-related research has surged during the decade following the previous survey by Fruehwirth. Covering more than 180 publications, this new survey provides an overview of recent results in a wide range of research areas, from semantics and analysis to systems, extensions and applications.

==> papers-plot.tex <==
%GNUPLOT: LaTeX picture with Postscript
\begin{picture}(0,0)%
\includegraphics{papers-plot}%
\end{picture}%
\begingroup
\setlength{\unitlength}{0.0200bp}%
\begin{picture}(18000,9719)(0,0)%
\put(1200,1200){\makebox(0,0)[r]{\strut{} 0}}%
\put(1200,2012){\makebox(0,0)[r]{\strut{} 5}}%
\put(1200,2824){\makebox(0,0)[r]{\strut{} 10}}%
\put(1200,3636){\makebox(0,0)[r]{\strut{} 15}}%
\put(1200,4448){\makebox(0,0)[r]{\strut{} 20}}%
\put(1200,5260){\makebox(0,0)[r]{\strut{} 25}}%
\put(1200,6072){\makebox(0,0)[r]{\strut{} 30}}%
\put(1200,6884){\makebox(0,0)[r]{\strut{} 35}}%
\put(1200,7696){\makebox(0,0)[r]{\strut{} 40}}%
\put(1200,8508){\makebox(0,0)[r]{\strut{} 45}}%
\put(1200,9320){\makebox(0,0)[r]{\strut{} 50}}%
\put(2477,800){\makebox(0,0){\strut{} 1998}}%
\put(4015,800){\makebox(0,0){\strut{} 1999}}%
\put(5554,800){\makebox(0,0){\strut{} 2000}}%
\put(7092,800){\makebox(0,0){\strut{} 2001}}%
\put(8631,800){\makebox(0,0){\strut{} 2002}}%
\put(10169,800){\makebox(0,0){\strut{} 2003}}%
\put(11708,800){\makebox(0,0){\strut{} 2004}}%
\put(13246,800){\makebox(0,0){\strut{} 2005}}%
\put(14785,800){\makebox(0,0){\strut{} 2006}}%
\put(16323,800){\makebox(0,0){\strut{} 2007}}%
\put(400,5260){\rotatebox{90}{\makebox(0,0){\strut{}Number of publications\ldots}}}%
\put(9400,200){\makebox(0,0){\strut{}Year}}%
\put(3100,8820){\makebox(0,0)[l]{\strut{}referring to \cite{fru_chr_overview_jlp98} {\tiny (source: Google Scholar)}}}%
\put(3100,8420){\makebox(0,0)[l]{\strut{}referred to in this survey, of which\ldots}}%
\put(3100,8020){\makebox(0,0)[l]{\strut{}\ldots from Melbourne/Singapore}}%
\put(3100,7620){\makebox(0,0)[l]{\strut{}\ldots from Leuven}}%
\put(3100,7220){\makebox(0,0)[l]{\strut{}\ldots from Germany}}%
\end{picture}%
\endgroup
\endinput

